Hierarchical Planning and Control for Box Loco-Manipulation

Humans perform everyday tasks using a combination of locomotion and manipulation skills. Building a system that can handle both skills is essential to creating virtual humans. We present a physically-simulated human capable of solving box rearrangement tasks, which requires a combination of both skills. We propose a hierarchical control architecture, where each level solves the task at a different level of abstraction, and the result is a physics-based simulated virtual human capable of rearranging boxes in a cluttered environment. The control architecture integrates a planner, diffusion models, and physics-based motion imitation of sparse motion clips using deep reinforcement learning. Boxes can vary in size, weight, shape, and placement height. Code and trained control policies are provided.

==> additional.tex <==
\section{Additional Results}

\subsection{Chest Juggling}

We also create a chest juggling skill, where the chest of the character is used to receive and bounce the ball. See Fig.~\ref{fig:teaser} for visualization.

\subsection{Foot Stalling}

Another common soccer juggling skill is foot stalling. To create a foot stalling skill, we create an additional control node called Right Foot Stall, or RFS. In the right foot stall, the reference motion is a fixed pose with the character standing on the left leg with the right leg lifted up, and the soccer ball lying still on top of the right foot. Directed edges from RFD to RFS and RFS to RFU are created to indicate transitions between them. To generate foot stalling motion with appropriate length, another edge connecting RFS to itself is also created. The weight of this self connected edge is set to be $30$ to indicate a desired longer duration of the stalling motion. See Fig.~\ref{fig:stall} for the control graph for generating a foot stall policy.

\begin{figure}
    \centering
    \includegraphics[width=0.5\columnwidth]{figures/stall.pdf}
    \caption{The control graph for creating a foot stall policy.}
    \label{fig:stall}
\end{figure}

\subsection{Foot Juggling with Different Heights}

For the foot juggling skill, we can randomize the desired traveling distance of ball $h$ in the vertical direction to train policy that can be capable of juggling the soccer ball at different heights. See Fig.~\ref{fig:height} for visualization.

\begin{figure}
    \centering
    \includegraphics[width=\columnwidth]{figures/height.pdf}
    \caption{We can generate a foot juggling policy that juggles the ball to different height.}
    \label{fig:height}
\end{figure}

==> low-level.tex <==
\section{Low-Level Control Policy}

Given the whole-body trajectory generated by the mid-level motion generator, we use reinforcement learning to train control policies to produce the desired motion in a physics-based simulation. We use RAISIM~\cite{raisim} to simulate the rigid body dynamics and Proximal Policy Optimization~\cite{ppo} to optimize the policies. The simulation frequency is \unit{120}{\hertz}, and the policy updates its output at \unit{60}{\hertz}.

\subsection{Policy Setup}
We represent our policy using a layer-wise mixture of experts neural network~\cite{2022-Soccer-Juggle}. The policy is tasked to track a reference motion that specifies the pose of the character over time. In particular, a reference motion of length $T$ is in the form of $\{ q^0_d, \cdots, q^{T-1}_d\}$, where $q^t_d$ includes the root linear position $p^t_d = \{p^t_{d, x}, p^t_{d, y}, p^t_{d, z}\}$ and root orientation $rot^t_d \in SO_3$ in the world frame, and the local joint rotation $j_d^t \in SO_3^{n_j}$. The input to the policy consists of the following data:

\begin{itemize}[leftmargin=\parindent]
    \setlength\itemsep{3pt}
    \item The state of the character. This includes the root height $p_z$, root linear and angular velocity $v_{\text{root}}, \omega_{{\text{root}}}$, and joint orientation $j$ and joint velocity $\dot{j}$. 
    \item Information about the next frame $q_d$ in the reference motion the policy needs to reach. This includes the deviation of the root linear position and root orientation from the reference motion ${p_{d, xy} - p_{xy}}, rot^d*rot^T$, and deviation of the joint orientation from the reference: $j_{d,i}*j_{i}^T$. All the information will be transformed into the local frame of the character.
\end{itemize}

An imitation-based reward is used to encourage the policy the track the reference motion. Specifically, three different reward terms are defined as follows:
\begin{align*}
    r_\text{joint} = &\exp(-3\|(\theta \ominus \theta_d)\|^2) \\
   r_\text{translation} = &\exp(-\|\dot{x} - \dot{x}_d \|^2 - \|\dot{y} - \dot{y}_d\|^2 - \|z - z_d\|^2)\\
   r_\text{orientation} = &\exp(-2\|o \ominus o_d \|^2),
\end{align*}
Following \cite{2019-siggraph-scadiver}, a total reward is calculated using the multiplication of these terms, i.e., at each time step, the policy receives a reward of $r = r_\text{joint} * r_\text{translation} * r_\text{orientation}$ to avoid the policy to ignore any of the reward terms.

The policy has enough information to track arbitrary reference motion capture data. Similar frameworks have been proposed in~\cite{2019-siggraph-drecon, 2019-siggraph-scadiver}. We adopt an action space where the control of the character is generated by a combination of Proportional-Derivative (PD) control and torque control, in particular, the torque applied in the simulation for each joint is generated via
\begin{align}
    \tau = k_p (j_{d} \ominus j) - k_d \dot{j} + \tau_{c},
\end{align}
where $k_p$ and $k_d$ are PD control gains and $\tau_{c}$ is a feedback torque generated by the policy to correct for errors that the naive PD control feedback fails to account for. This is inspired by \cite{2022-Soccer-Juggle}.

\subsection{Locomotion Policy}
Our locomotion policy is trained by imitating motion capture data of a human walking around in various directions at various speeds. The motion capture data is taken from~\cite{2019-TOG-neural_state_machine}. At the beginning of each episode during training, a motion sequence is sampled randomly from the dataset, the character is initialized to the state of the first frame of the sampled sequence. A total of $89395$ frames (approximately $25$ minutes) of data are being used for training. 

\subsection{Locomotion while Carrying Boxes}
We augment the locomotion dataset by fixing the arm motion to be in a fixed pose that corresponds to a carrying pose. During training, we initialize the box to be directly in front of the character between the two hands. In addition to the standard imitation-based reward, the policies also receive a reward for placing the hand on the side of the box and keeping the box orientation to be always the default orientation in the character frame. Specifically, the box related reward is calculated via

\begin{align*}
    r_\text{box-orientation} = &\exp(-10\|(\theta_\text{box} \ominus \theta_{d, \text{box}})\|^2) \\
   r_\text{box-hand} = &\exp(-\| p_{lhand} - p_{lbox}\|^2 - \| p_{rhand} - p_{rbox}\|^2)\\
\end{align*}

A total reward of $r_\text{ball1} = r_\text{box-orientation} + r\text{ball-hand}$ is computed at each time step. We also create scenarios where the character is tasked to carry two boxes. Additional rewards 
\begin{align*}
    r_\text{box2-orientation} = &\exp(-10\|(\theta_\text{box2} \ominus \theta_{d, \text{box2}})\|^2) \\
   r_\text{box2-position} = &\exp(-\| p_{box1} - p_{box2}\|^2)\\
\end{align*}
are calculated, where $r_\text{box2-orientation}$ penalize deviation of the box orientation to a default orientation in the character frame, and $r_\text{box2-position}$ penalize deviation of the box position relative to the bottom box location. A final reward $r_\text{box} = r_\text{box1} * r_\text{box2-orientation} * r_\text{box2-orientation}$. Additional boxes can also be added by computing the orientation and position reward similarly and multiply them with $r_\text{box}$.

\subsection{Pick Up and Place Down Policy}

==> mid_level.tex <==
\section{Mid-Level Whole-Body Pose Generator}
We use diffusion model \cite{diffusion} to generate whole-body pose sequences to navigate in environment. The diffusion model is trained with the locomotion dataset from \cite{2019-TOG-neural_state_machine}.

\subsection{Diffusion Model}
The diffusion model aims to recover a full-body pose sequence from a noisy input via a iterative denoising process. During training, noise is added to the data and a denoising model is trained to recover the original data from the noisy data.

==> notes.tex <==
\section{System Overview}
Our system aims to generate animations of a physically simulated character arranging the boxes by picking them up, carrying them, and putting them down while navigating the 3D scene to achieve the desired configuration for those boxes. Figure \ref{fig:system} shows the overview of our system. 

Rearrangement tasks in a contextual environment requires coordinated locomotion and manipulation which can be broken down to four primitive motions: walk-only without objects, walk-and-carry objects, pick-up objects, and put-down objects. We construct a simple graph to express the sequential relationships among those primitives: an arrow from primitive A to B indicates that B can be executed after A but not vice versa (Figure \ref{fig:system} middle part).

The high-level planner takes as input the desired arrangement of the boxes and the 3D scene and plans a primitive path on the graph to achieve the desired box arrangement. If the path contains locomotion primitives, i.e. Walk-only and Walk-and-carry, the planner will also generate waypoints for each locomotion primitive to avoid collisions in the scene. 

Once planned, each motion primitive generates or retrieves kinematic reference motion and executes its low-level policy to track the reference motion via physics simulation. For the locomotion primitives, we leverage a large-scale mocap dataset and train a diffusion model to generate various walking motion to navigate the scene, conditioned on the waypoints. Simple tracking policies are then used to track the kinematic walking motion generated by the diffusion model. For the manipulation primitives, i.e. Pick-up and Put-down, we only use a single reference trajectory and rely on a more powerful manipulation policy to achieve a wide variety of tasks.


%We model the character as an articulated rigid body system, adapted from Scadiver \cite{2019-siggraph-scadiver}. It has $59$ degrees of freedom, including a floating base. We use RAISIM~\cite{raisim} as the physics simulator. The character is controlled via Stable proportional-derivative controllers~\cite{2011-StablePD}. 

% An overview of our system is shown in Fig.~\ref{fig:system}.
% A motion generator is used to generate a whole-body trajectory that respects user-specified root position and orientation. A control policy, trained with reinforcement learning, takes this whole-body trajectory and tries to reproduce this trajectory in a physics simulator while manipulating the objects to move with the character.

